Predicting Stochastic Human Forward Reachable Sets Based on Learned Human Behavior

With the recent surge of interest in introducing autonomous vehicles to the everyday lives of people, developing accurate and generalizable algorithms for predicting human behavior becomes highly crucial. Moreover, many of these emerging applications occur in a safety-critical context, making it even more urgent to develop good prediction models for human-operated vehicles. This is fundamentally a challenging task as humans are often noisy in their decision processes. Hamilton-Jacobi (HJ) reachability is a useful tool in control theory that provides safety guarantees for collision avoidance. In this paper, we first demonstrate how to incorporate information derived from HJ reachability into a machine learning problem which predicts human behavior in a simulated collision avoidance context, and show that this yields a higher prediction accuracy than learning without this information. Then we propose a framework to generate stochastic forward reachable sets that flexibly provides different safety probabilities and generalizes to novel scenarios. We demonstrate that we can construct stochastic reachable sets that can capture the trajectories with probability from 0.75 to 1.

==> formulation.tex <==
% !TEX root = MIP.tex
\section{Problem Formulation \label{sec:formulation}}
Consider $N$ vehicles, denoted $\veh_i, i = 1, 2, \ldots, N$, described by the following ordinary differential equation (ODE)
\vspace{-0.75em}
\begin{equation}
\label{eq:vdyn} % vehicle dynamics
\dot{x}_i = f_i(x_i, u_i), \quad u_i \in \cset_i, \quad i = 1,\ldots, N
\end{equation}

\noindent where $x_i \in \R^{n_i}$ is the state of the $i$th vehicle $\veh_i$, and $u_i$ is the control of $\veh_i$. Each of the $N$ vehicles may have some objective, such as getting to a set of goal states. Whatever the objective may be, each vehicle $\veh_i$ must at all times avoid the \textit{danger zone} $\dz_{ij}$ with respect to each of the other vehicles $\veh_j, j = 1, \ldots, N, j \neq i$. In general, the danger zones $\dz_{ij}$ may represent any relative configuration between $\veh_i$ and $\veh_j$ that are considered undesirable, such as collision. In this paper, we make the assumption that $x_i \in \dz_{ij} \Leftrightarrow x_j \in \dz_{ji}$, the interpretation of which is that between a pair of vehicles, an unsafe configuration is one in which either of the vehicle is the danger zone of the other.

If possible and desired, each vehicle would use a ``liveness controller'' that helps complete its objective. However, sometimes a ``safety controller'' must be used in order to prevent the vehicle from entering any danger zones with respect to any other vehicles. Since the danger zones $\dz_{ij}$ are sets of joint configurations, it is convenient to derive the set of relative dynamics between every vehicle pair from the dynamics of each vehicle specified in $\eqref{eq:vdyn}$. Let the relative dynamics between $\veh_i$ and $\veh_j$ be specified by the ODE
\vspace{-0.5em}
\begin{equation}
\label{eq:rdyn} % relative dynamics
\begin{aligned}
\dot{x}_{ij} &= g_{ij}(x_{ij}, u_i, u_j) \\
u_i &\in \cset_i, u_j \in \cset_j \quad i, j = 1, \ldots, N, i\neq j 
\end{aligned}
\end{equation}

We assume the functions $f_i$ and $g_{ij}$ are uniformly continuous, bounded, and Lipschitz continuous in arguments $x_i$ and $x_{ij}$ respectively for fixed $u_i$ and $(u_i, u_j)$ respectively. In addition, the control functions $u_i(\cdot)\in\cfset_i$ are drawn from the set of measurable functions\footnote{A function $f:X\to Y$ between two measurable spaces $(X,\Sigma_X)$ and $(Y,\Sigma_Y)$ is said to be measurable if the preimage of a measurable set in $Y$ is a measurable set in $X$, that is: $\forall V\in\Sigma_Y, f^{-1}(V)\in\Sigma_X$, with $\Sigma_X,\Sigma_Y$ $\sigma$-algebras on $X$,$Y$.}.

Given the vehicle dynamics in \eqref{eq:vdyn}, some joint objective, the derived relative dynamics in \eqref{eq:rdyn}, and the danger zones $\dz_{ij}, i,j = 1, \ldots, N, i \neq j$, we propose a cooperative safety control strategy that performs the following:

\begin{enumerate}
\item detect potential conflict based on the joint configuration of all $N$ vehicles;
\item allow vehicles that are not in potential conflict to complete their objective using a liveness controller;
\item among the vehicles in potential conflict, attempt to minimize the number of instances in which a vehicle gets into another vehicle's danger zone.
\end{enumerate}

For the case of $N=3$, we prove that our proposed control strategy guarantees that all vehicles will be able to stay out of all the danger zones with respect to the other vehicles, and thus guaranteeing safety. For all initial configurations in our simulations, all vehicles also complete their objectives.


==> main_result.tex <==
% !TEX root = MIP.tex
\section{Safety Guarantee For Three Vehicles}
The method for constructing a joint safety controller described in Section \ref{eq:method} guarantees safety when $N = 3$. We now formally states this guarantee and prove the result.

\begin{thm}
\label{thm:main_result}
Suppose $N = 3$. If $\sv_{12}, \sv_{23}, \sv_{31} \ge 0$ at some time $t = t_0$, then the joint control strategy from the MIP \eqref{eq:baseMIP} with the reward coefficient matrix elements $\rcm_{ij}$ chosen in Section \ref{sec:Rcm} guarantees that $\sv_{12}, \sv_{23}, \sv_{31} \ge 0 ~ \forall t > t_0$.
\end{thm}

\begin{proof}
It suffices to show that $0 \le \sv_{12}, \sv_{23}, \sv_{31} \le \st$ at $t = t_0$ implies $\sv_{12}, \sv_{23}, \sv_{31} \ge 0 ~ \forall t > t_0$.

Suppose $0 \le \sv_{12} \le \st$. Then $\rcm_{12} = 36$. From the objective of \eqref{eq:baseMIP}, $\ulo_{12}$ would be chosen to be $1$ unless another feasible solution in which $\ulo_{12} = 0$ results in a higher objective value. Due to (\ref{eq:baseMIP}a) and (\ref{eq:baseMIP}b), the only way for the optimal solution to have $\ulo_{12} = 0 $ is to have $\ulo_{13} = 1$ or $\ulo_{21} = 1$.

There are several cases of $\Rcm$ to go through, with each case having different elements of $\Rcm$ being equal to $-1$. We show one case here; the rest of the cases follow a similar logic. Assume $\Rcm$ is given in \eqref{eq:Rcmfull}. Then, since $\rcm_{ij} > 0 ~ \forall i,j,i\neq j$, the optimal solution would have as many elements of $\Ulo$ being $1$ as possible (except for diagonal elements).

Suppose $\ulo_{21} = 1$, then by (\ref{eq:baseMIP}a), $\ulo_{12} = 0$ and by (\ref{eq:baseMIP}b), $\ulo_{23} = 0$. This leaves us with the freedom to choose $\ulo_{13}, \ulo_{31}, \ulo_{32}$. Since $\Rcm_{31} = 16 > 9 + 1 = \Rcm_{13} + \Rcm_{32}$, choosing $\ulo_{31} = 1, \ulo_{13} = \ulo_{32} = 0$ would maximize the objective. This gives us the candidate solution $\ulo_{21}=1, \ulo_{31} = 1$ and the rest of the $\ulo_{ij}$ being $0$, with an objective value of $4 + 16 = 20$. However, choosing $\ulo_{12} = 1$ alone would already result in an objective value of at least $\Rcm_{12} = 36$; therefore, $\ulo_{21} \neq 1$.

Next, suppose $\ulo_{13} = 1$, then by (\ref{eq:baseMIP}a), $\ulo_{12} = 0$ and by (\ref{eq:baseMIP}b), $\ulo_{31} = 0$. This leaves us with the freedom to choose $\ulo_{21}, \ulo_{23}, \ulo_{32}$. Since $\Rcm_{23} = 25 > 4 + 1 = \Rcm_{21} + \Rcm_{32}$, choosing $\ulo_{23} = 1, \ulo_{21} = \ulo_{32} = 0$ would maximize the objective. This gives us the candidate solution $\ulo_{13}=1, \ulo_{23} = 1$ and the rest of the $\ulo_{ij}$ being $0$, with an objective value of $9 + 25 = 34$. However, choosing $\ulo_{12} = 1$ alone would already result in an objective value of at least $\Rcm_{12} = 36$; therefore, $\ulo_{13} \neq 1$.

This leaves us with $\ulo_{12} = 1$ whenever $0 \le \sv_{12} \le \st$. By a similar argument, one can show that $\ulo_{23} = 1$ whenever $0 \le \sv_{23} \le \st$, and $\ulo_{31} = 1$ whenever $0 \le \sv_{31} \le \st$.
\end{proof}

\begin{rmk}
Alternatively, one could enumerate all feasible solutions for every possible choice of $\Rcm$, and discover the same result stated in Theorem \ref{thm:main_result}. We have also taken this brute force approach to verify the above proof.
\end{rmk}

\begin{corr}
By Theorem \ref{thm:main_result} and Corollary \ref{corr:pw_safety}, if $N = 3$ and each vehicle $\veh_i$ uses the optimal pairwise safety controller $u_{ij}^*$ with respect to $\veh_j$ whenever $\ulo_{ij} = 1$, then no vehicle will ever get into another vehicle's danger zone.
\end{corr}

